Explanations of Black-Box Models based on Directional Feature Interactions

As machine learning algorithms are deployed ubiquitously to a variety of domains, it is imperative to make these often black-box models transparent. Several recent works explain black-box models by capturing the most influential features for prediction per instance; such explanation methods are univariate, as they characterize importance per feature. We extend univariate explanation to a higher-order; this enhances explainability, as bivariate methods can capture feature interactions in black-box models, represented as a directed graph. Analyzing this graph enables us to discover groups of features that are equally important (i.e., interchangeable), while the notion of directionality allows us to identify the most influential features. We apply our bivariate method on Shapley value explanations, and experimentally demonstrate the ability of directional explanations to discover feature interactions. We show the superiority of our method against state-of-the-art on CIFAR10, IMDB, Census, Divorce, Drug, and gene data.

==> append/limitation.tex <==


\begin{appendices}




\section{Limitation}

\label{app:limitation}


Interpretation is subjective making evaluations of results difficult.
%, the ambiguity its meaning makes the evaluation hard. 
Here we evaluate our result through a known metric called post-hoc accuracy \citeapp{pmlr-v80-chen18j}, which tracks the changes in the output of a black box via the changes of its input. 
Further research on developing additional objective quantitative measures for interpretation are needed.
Evaluating interpretations also depend on the context and the application the black-box model will be utilized.  In this paper, 
we investigate the result of the most influential gene data for smokers and non-smokers by investigating its correspondence with known influential genes the Gene Ontology (GO) knowledgebase.
%from biology literature known as the GO category. 
This is one possible check of the quality of the results.  Ultimately, in a discovery task, such as this work, we need to further investigate these results through carefully designed biology experiments.
Our theoretical result, Corollary~\ref{'cor:transitivity'}, proves the ideal case of of transitivity defined in Def \ref{'def:transitivity'} in graph $\mathcal{H}$. However
Thm.~\ref{'thm: upper bound triangulation inequality '} proves `almost transitivity' in the general for approximation graph $\mathcal{H}^{\gamma}$.
 Moreover, our experiments show the effectiveness of our method even when these assumptions are violated.
%However, the ambiguity of interpretation makes it hard to evaluate the result beyond that. Furthermore, the results of theorem corollary $\ref{'cor:transitivity'}$ is proven in the ideal case. However, the theorem $\ref{'thm: upper bound triangulation inequality '}$ introduces the relation in the approximation case. In addition, we show the effectiveness of our method in the relaxed cases.






    
\end{appendices}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/table_AUC_iclr_revisions.tex <==



\begin{table*}[t]
\scriptsize
\centering
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|c| c c c c c c c|c c c c c c c|}
    \hline
    & \multicolumn{7}{|c|}{Insertion AUC (Higher is better)}  & 
    \multicolumn{7}{|c|}{Deletion AUC (Lower is better)} \\
	\hline
    
	\hline
	Dataset &
	    COPD&
	    CIFAR10& 
		MNIST&
		IMDB&
		Census&
		Divorce&
	    Drug&
	    COPD&
	    CIFAR10& 
		MNIST&
		IMDB&
		Census&
		Divorce&
	    Drug&
		\hline 
		
	Ours-SS &
		0.48 &
		0.75 &
		0.85 &
		0.45 &
		0.43 &
		0.30 &
		0.30 &
		0.01&
		0.05&
		0.03&
		0.02&
		0.32&
		0.05&
		0.10&
		
	Ours-K &
		0.49 &
		0.65 &
		0.84 &
		0.43 &
		0.42 &
		0.30 &
		0.30 &
		0.00 &
		0.08 &
		0.03&
		0.02 &
		0.32 &
		0.05 &
		0.10 &
		
	Sh-Sam&
		0.48 &
		0.75 &
		0.85 &
		0.45 &
		0.43 &
		0.30 &
		0.30 &
		0.01 &
		0.05 &
		0.03&
		0.02 &
		0.32 &
		0.05 &
		0.10 &
		
	kSHAP &
		0.42 &
		0.48 &
		0.77 &
		0.29 &
		0.42 &
		0.29 &
		0.30 &
		0.09 &
		0.17 &
		0.17 &
		0.03 &
		0.36 &
		0.05 &
		0.11 &
		
	Sh-Int &
		0.20 &
		0.35 &
		0.46 &
		0.32 &
		0.43 &
		0.16 &
		0.17 &
		0.23 &
		0.31 &
		0.52 &
		0.29 &
		0.33 &
		0.14 &
		0.20 &
		
	Sh-Tay &
		-- &
		0.34 &
		0.78 &
		0.34 &
		0.06 &
		0.17 &
		0.29 &
		-- &
		0.27 &
		0.19 &
		0.19 &
		0.06 &
		0.10 &
		0.11 &
		
		
	Sh-Exc &
		-- &
		0.32 &
		0.51 &
		0.30 &
		0.37 &
		0.15 &
		0.08 &
		-- &
		0.31 &
		0.48 &
		0.29 &
		0.38 &
		0.15 &
		0.29 &
		
		
	GNNExp &
		0.25 &
		0.15 &
		0.25 &
		0.30 &
		0.38 &
		0.25 &
		0.26 &
		0.25 &
		0.15 &
		0.25 &
		0.30 &
		0.38 &
		0.25 &
		0.27 &

		
	\hline
\end{tabular}
\caption{Influential Feature Evaluation through Insertion and Deletion AUC. We calculate a feature ranking by applying PageRank on the $\mathcal{G}$ graph, iteratively removing the most influential feature, then evaluating AUC on the resulting curve. Note that we cannot run Sh-Tay and Sh-Exc methods on the COPD dataset due to their computational issues with the large number of features.}
\label{table:AUC}
\end{table*}


\iffalse
\begin{table*}[t]
\scriptsize
\centering
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|c| c c c c c c|c c c c c c|}
    
	\hline
	Dataset &
	    Ours (SS)&
	    Ours (K) & 
		Sh-Samp &
		KernelSHAP &
		Sh-Int &
		Sh-Excess &
	    Ours (SS)&
	    Ours (K) & 
		Sh-Samp &
		KernelSHAP &
		Sh-Int &
		Sh-Excess &
		\hline 
		
	COPD &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		
	CIFAR10 &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		
	MNIST &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
	IMDB &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		
	Census &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		
	Divorce &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		
	Drug &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &

		
		
		

	\hline
\end{tabular}
\caption{Caption}
\label{table:AUC}
\end{table*}
\fi

==> tables/table_AUC_rev1.tex <==


\begin{table*}[t]
\scriptsize
\centering
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{| l | c| c c c c c c c|c c c c c c c|}
    \hline
    & & \multicolumn{7}{|c|}{\textbf{Insertion AUC} $\uparrow$}  & 
    \multicolumn{7}{|c|}{ \textbf{Deletion AUC} $\downarrow$} \\
	\hline
    
	\hline
	Order & 
	Method &
	    COPD&
	    CIFAR10& 
		MNIST&
		IMDB&
		Census&
		Divorce&
	    Drug&
	    COPD&
	    CIFAR10& 
		MNIST&
		IMDB&
		Census&
		Divorce&
	    Drug&
		\hline 
		
	Bivariate &
	Ours-SS &
		49.1 &
		57.3 &
		81.4 &
		43.7 &
		11.5 &
		30.4 &
		30.1 &
		0.1&
		17.1&
		7.5&
		1.8&
		1.7&
		4.8&
		10.4&
	&	
	Ours-K &
		49.0 &
		66.1 &
		84.1 &
		43.5 &
		11.5 &
		30.4 &
		30.1 &
		0.2 &
		8.4 &
		3.2 &
		1.9 &
		1.7 &
		4.8 &
		10.4 &
	&	
	Sh-Int &
		26.8 &
		??? &
		47.1 &
		19.6 &
		8.2 &
		24.7 &
		17.4 &
		23.6 &
		?? &
		51.2 &
		20.1 &
		4.4 &
		8.3 &
		20.0 &
	&	
	Sh-Taylor &
		-- &
		-- &
		-- &
		-- &
		6.8 &
		15.1 &
		9.3 &
		-- &
		-- &
		-- &
		-- &
		4.8 &
		13.5 &
		30.0 &
	&	
	Sh-Exc &
		-- &
		-- &
		-- &
		-- &
		6.8 &
		15.1 &
		9.3 &
		-- &
		-- &
		-- &
		-- &
		4.8 &
		13.5 &
		30.0 &
	    \hline
	Univariate &	
	Sh-Sam&
		48.6 &
		57.6 &
		81.4 &
		43.7 &
		11.5 &
		30.4 &
		30.0 &
		0.2 &
		17.0 &
		7.7 &
		1.8 &
		1.7 &
		4.8 &
		10.4 &
	&	
	kSHAP &
		48.9 &
		60.9 &
		83.6 &
		43.0 &
		9.1 &
		30.2 &
		30.0 &
		0.2 &
		14.6 &
		3.8 &
		2.1 &
		2.0 &
		4.9 &
		10.4 &
	&	
	L2X&
	    ?? &
	    ?? &
	    ?? &
	    ?? &
	    ?? &
	    ?? &
	    ?? &
	    ?? &
	    ?? &
	    ?? &
	    ?? &
	    ?? &
	    ?? &
	    ?? &
		
		

	\hline
\end{tabular}
\caption{Caption}
\label{table:compare}
\end{table*}


\iffalse
\begin{table*}[t]
\scriptsize
\centering
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|c| c c c c c c|c c c c c c|}
    
	\hline
	Dataset &
	    Ours (SS)&
	    Ours (K) & 
		Sh-Samp &
		KernelSHAP &
		Sh-Int &
		Sh-Excess &
	    Ours (SS)&
	    Ours (K) & 
		Sh-Samp &
		KernelSHAP &
		Sh-Int &
		Sh-Excess &
		\hline 
		
	COPD &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		
	CIFAR10 &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		
	MNIST &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
	IMDB &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		
	Census &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		
	Divorce &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		
	Drug &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &

		
		
		

	\hline
\end{tabular}
\caption{Caption}
\label{table:compare}
\end{table*}
\fi

==> tables/table_AUC_rev2.tex <==

\begin{table*}[t]
\scriptsize
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.2}
\subfloat[caption]{
\begin{tabular}{|c| c c c c c | c c c|}
    \hline
    & \multicolumn{5}{|c|}{Bivariate Methods}  & 
    \multicolumn{3}{|c|}{Univariate Methods} \\
    
	\hline
	Dataset &
	    Our-SS&
	    Ours-K& 
		Sh-Int&
		Sh-Tay&
		Sh-Exc&
		Sh-Sam&
		kSHAP&
		L2X&
		\hline 
		
	COPD &
		5940 &
		35.7 &
		2880 &
		??? &
		??? &
		5810 &
		1.37 &
		-- &
		
	CIFAR10 &
		218 &
		2.54 &
		??? &
		??? &
		??? &
		223 &
		0.652 &
		-- &
		
	MNIST &
		116 &
		1.46 &
		47.9 &
		??? &
		??? &
		116 &
		0.344 &
		-- &
	IMDB &
		207 &
		1.94 &
		160 &
		??? &
		??? &
		104 &
		0.403 &
		-- &
		
	Census &
		2.71 &
		0.202 &
		2.58 &
		2.58 &
		5.30 &
		2.16 &
		0.826 &
		-- &
		
	Divorce &
		18.2 &
		0.337 &
		6.48 &
		93.3 &
		93.3 &
		22.1 &
		0.156 &
		-- &
		
	Drug &
		2.34 &
		0.07 &
		1.22 &
		1.22 &
		0.960 &
		3.99 &
		0.097 &
		-- &

		
		
		

	\hline
\end{tabular}
}
\quad 
\subfloat[We use PageRank to identify $\mathcal{H}$-sink and $\mathcal{H}$-source nodes. $\mathcal{H}$-sink nodes represent directional redundancy with respect to $\mathcal{H}$-source nodes; we see a minimal decrease in accuracy when masking the redundant $\mathcal{H}$-sink nodes nodes.]{
\begin{tabular}{| p{1.3cm} p{1.3cm} | p{1.3cm} p{1.3cm} |}
    \hline
    \multicolumn{2}{|c|}{PH-Accy}  & 
    \multicolumn{2}{|c|}{\% Feat Masked} \\
    
	\hline
		
		$\mathcal{H}$-Sink Masked & 
		$\mathcal{H}$-Source  Masked &
		$\mathcal{H}$-Sink Masked & 
		$\mathcal{H}$-Source Masked &
		
    	\hline
	
		99.5&
		62.7&
		1.5 &
		98.5 &
		
		94.6 &
		15.0 &
		6.2 &
		93.8 &
		
		100.0 &
		13.4 &
		77.7 &
		22.3 &
		
		100.0 &
		54.0 &
		3.5 &
		96.5 &
		
		100.0 &
		82.0 &
		23.8 &
		76.2 &
		
		100.0 & 
		51.5 & 
		22.2 & 
		77.8 & 
		
		100.0 & 
		48.5 & 
		43.5 & 
		56.5 & 

		
		
		

	\hline
\end{tabular}
}
\end{table*}

==> tables/table_AUC_rev3.tex <==
\begin{table*}[t]
\scriptsize
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.2}

\begin{minipage}{.5\linewidth}
        \centering
          
          
        \begin{tabular}{|c| c c c c c | c c c|}
            \hline
            & \multicolumn{5}{|c|}{Bivariate Methods}  & 
            \multicolumn{3}{|c|}{Univariate Methods} \\
            
        	\hline
        	Dataset &
        	    Our-SS&
        	    Ours-K& 
        		Sh-Int&
        		Sh-Tay&
        		Sh-Exc&
        		Sh-Sam&
        		kSHAP&
        		L2X&
        		\hline 
        		
        	COPD &
        		0.48 &
        		0.49 &
        		0.20 &
        		* &
        		* &
        		0.48 &
        		0.42 &
        		-- &
        		
        	CIFAR10 &
        		0.75 &
        		0.65 &
        		0.35 &
        		* &
        		* &
        		0.75 &
        		0.48 &
        		-- &
        		
        	MNIST &
        		0.85 &
        		0.84 &
        		0.46 &
        		* &
        		* &
        		0.85 &
        		0.77 &
        		-- &
        	IMDB &
        		0.45 &
        		-- &
        		0.32 &
        		* &
        		* &
        		0.45 &
        		0.29 &
        		-- &
        		
        	Census &
        		0.43 &
        		0.202 &
        		2.58 &
        		2.58 &
        		5.30 &
        		2.16 &
        		0.826 &
        		-- &
        		
        	Divorce &
        		18.2 &
        		0.337 &
        		6.48 &
        		93.3 &
        		93.3 &
        		22.1 &
        		0.156 &
        		-- &
        		
        	Drug &
        		2.34 &
        		0.07 &
        		1.22 &
        		1.22 &
        		0.960 &
        		3.99 &
        		0.097 &
        		-- &
        
        		
        		
        		
        
        	\hline
        \end{tabular}
    \caption{Influential Feature Evaluation through Deletion AUC. We calculate a feature ranking by applying PageRank on the $\mathcal{G}$ graph, iteratively removing the most influential feature, then evaluating AUC on the resulting curve. Note that Sh-Tay and Sh-Exc were only evaluated on the simpler datasets Census, Divorce, and Drug due to computational complexity.}
    \end{minipage}%

\begin{minipage}{.5\linewidth}
      \centering
      
    \begin{tabular}{| p{0.8cm} p{0.8cm} | p{0.8cm} p{0.8cm} |}
        \hline
        \multicolumn{2}{|c|}{PH-Accy}  & 
        \multicolumn{2}{|c|}{\% Feat Masked} \\
        
    	\hline
    		
    		Sink Masked & 
    		Source Masked &
    		Sink Masked & 
    		Source Masked &
    		
        	\hline
    	
    		99.5&
    		62.7&
    		1.5 &
    		98.5 &
    		
    		94.6 &
    		15.0 &
    		6.2 &
    		93.8 &
    		
    		100.0 &
    		13.4 &
    		77.7 &
    		22.3 &
    		
    		100.0 &
    		54.0 &
    		3.5 &
    		96.5 &
    		
    		100.0 &
    		82.0 &
    		23.8 &
    		76.2 &
    		
    		100.0 & 
    		51.5 & 
    		22.2 & 
    		77.8 & 
    		
    		100.0 & 
    		48.5 & 
    		43.5 & 
    		56.5 & 
    
    		
    		
    		
    
    	\hline
    \end{tabular}
    \caption{Directional Redundancy Evaluation. We compare Posthoc-accuracy after masking $\mathcal{H}$-source nodes, which represent features containing minimal redundancies, and $\mathcal{H}$-sink nodes, which represent directionally redundant features. We see a minimal decrease in accuracy when masking the redundant $\mathcal{H}$-sink nodes nodes.}
    \label{tab:directional_redundancy}
\end{minipage}%
\end{table*}


%\subfloat[We use PageRank to identify $\mathcal{H}$-sink and $\mathcal{H}$-source nodes. $\mathcal{H}$-sink nodes represent directional redundancy with respect to $\mathcal{H}$-source nodes; we see a minimal decrease in accuracy when masking the redundant $\mathcal{H}$-sink nodes nodes.]

==> tables/table_COPD_rev0.tex <==


\begin{table*}[t]
\scriptsize
\centering
%\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1}



\begin{tabular}{|l|l|c|c|}
    \hline

	\textbf{Group} &
		\textbf{Pathway Name} &
		\textbf{Genes} &
		\textbf{q-value} &

		\hline 
	Smoker &
		\textbf{GSE25123\_WT\_VS\_PPARG\_KO\_MACROPHAGE\_IL4\_STIM\_DN} &
		\textbf{23} &
		\textbf{0.02} &


	 &
		GSE32986\_GMCSF\_VS\_GMCSF\_AND\_CURDLAN\_LOWDOSE\_STIM\_DC\_UP &
		24 &
		0.16 &

	 &
		GSE45365\_WT\_VS\_IFNAR\_KO\_CD11B\_DC\_UP &
		18 &
		0.20 &

        \hline
	 NonSmoker &
		\textbf{GSE25123\_WT\_VS\_PPARG\_KO\_MACROPHAGE\_IL4\_STIM\_DN} &
		\textbf{23} &
		\textbf{0.01} &

	 &
		GSE32986\_UNSTIM\_VS\_CURDLAN\_LOWDOSE\_STIM\_DC\_DN &
		28 &
		0.13 &

	 &
		GSE32986\_GMCSF\_VS\_GMCSF\_AND\_CURDLAN\_LOWDOSE\_STIM\_DC\_UP &
		24 &
		0.21 &


	\hline
\end{tabular}
\caption{GO enrichment results for the redundancy-based ranking of graph $\mathcal{G}$ for Smoker and Nonsmoker subgroups. Gene pathways with q-value $<0.05$ are bolded.}
\label{table:COPD}
\end{table*}



==> tables/table_TimeComplexity.tex <==
\begin{table*}[t]
%------------------------------------------
\scriptsize
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.2}
\centering
\begin{tabular}{|c| c| c c c c c | c c c| c|}
    \hline
    & & \multicolumn{5}{|c|}{Bivariate Methods}  & 
    \multicolumn{3}{|c|}{Univariate Methods} & GNN Methods \\
    
	\hline
	Dataset &
	    \# Features &
	    Ours-SS&
	    Ours-K& 
		Sh-Int&
		Sh-Tay & 
		Sh-Exc&
		Sh-Sam&
		kSHAP&
		L2X&
		GNNExp&
		\hline 
		
	COPD &
	1077 &
		5942 &
		36 &
		2877 &
		112900 &
		838200 &
		3047 &
		1.4 &
		0.00 &
		10.9 &
		
	CIFAR10 &
	255 &
		218 &
		2.5 &
		101 &
		2819 &
		6267 &
		140 &
		0.65 &
		0.00 &
		0.79 &
		
	MNIST &
	196 &
		116 &
		1.5 &
		48 &
		1194 &
		2350 &
		57 &
		0.34 &
		0.00 &
		0.42 &
		
	IMDB &
	$\leq$400 &
		207 &
		1.9 &
		160 &
		1279 &
		1796 &
		103 &
		0.40 &
		0.00 &
		0.73 &
		
	Census &
	12 &
		2.7 &
		0.20 &
		2.6 &
		11.6 &
		5.3 &
		1.6 &
		0.83 &
		0.00 &
		0.17 &
		
	Divorce &
	54 &
		18.2 &
		0.34 &
		6.5 &
		63.2 &
		93.3 &
		11.3 &
		0.16 &
		0.00 &
		0.15 &
		
	Drug &
	6 &
		2.3 &
		0.07 &
		1.21 &
		181 &
		0.96 &
		1.26 &
		0.10 &
		0.00 &
		1.54 &

		
		
		

	\hline
\end{tabular}
\caption{Time comparisons of the methods. Results are calculated on the time to produce the interaction matrix (including all features) for a single sample, as measured by seconds per sample.}
\label{table:time}

\end{table*}



\iffalse
\begin{table*}[t]
%------------------------------------------
\scriptsize
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.2}
\centering
        \begin{tabular}{|c| c| c c c c c |}
            \hline
            \multicolumn{7}{|c|}{Time Complexity: Seconds per Sample}  \\
            
        	\hline
        	Dataset &
        	    \#Features &
        	    BivShap-S&
        	    BivShap-K& 
        		Sh-Int&
        		Sh-Tay & 
        		Sh-Exc&
        		\hline 
        		
        	COPD &
        	1077 &
        		5942 &
        		36 &
        		2877 &
        		112900 &
        		838200 &
        		
        	CIFAR10 &
        	255 &
        		218 &
        		2.5 &
        		101 &
        		2819 &
        		6267 &
        		
        	MNIST &
        	196 &
        		116 &
        		1.5 &
        		48 &
        		1194 &
        		2350 &
        		
        	IMDB &
        	$\leq$400 &
        		207 &
        		1.9 &
        		160 &
        		1279 &
        		1796 &
        		
        	Census &
        	12 &
        		2.7 &
        		0.20 &
        		2.6 &
        		11.6 &
        		5.3 &
        		
        	Divorce &
        	54 &
        		18.2 &
        		0.34 &
        		6.5 &
        		63.2 &
        		93.3 &
        		
        	Drug &
        	6 &
        		2.3 &
        		0.07 &
        		1.21 &
        		10.1 &
        		0.96 &
        
        	\hline
        \end{tabular}
       \setlength{\belowcaptionskip}{-10}
      
      \caption{Time comparisons of the methods. Results are calculated on the time to produce the interaction matrix (including all features) for a single sample, as measured by seconds per sample.}
    \label{table:time}
\end{table*}
\fi

==> tables/table_redundancy.tex <==


\begin{figure}
  \begin{minipage}[b]{0.6\linewidth}
    \centering
    \includegraphics[width=1.3\linewidth]{NeuRIPS2019/figures/MR.png}
  \end{minipage}%
  \begin{minipage}[b]{0.01\linewidth}
    \centering
    
    %=======================        
    \begin{tabular}{|c|c|c|}
        \hline
    
    	\textbf{Dataset} &
    		\textbf{Sink Masked} &
    		\textbf{Source Masked} &
    
    		\hline 
    	COPD &
    		0.000 &
    		-- &
    
    		\hline 
    	CIFAR10 &
    		0.000 &
    		-- &
    		\hline 
    	MNIST &
    		0.000 &
    		-- &
    		\hline 	 
    	IMDB &
    		0.000 &
    		-- &
    		\hline 	 
    	Census &
    		0.000 &
    		-- &
    		\hline 	 
    	Divorce &
    		0.000 &
    		-- &
    		\hline 	 
    	Drug &
    		0.000 &
    		-- &
    		\hline 	 		
    
    	\hline
    \end{tabular}
    %=======================
\end{minipage}
\caption{Caption}
\label{fig:test}
\end{figure}


==> tables/table_redundancy_v1.tex <==




\begin{table*}[t]
\scriptsize
\centering
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|l c||c|c||c|c||c|c|c||c|c|c||}
    \hline
    & & \multicolumn{2}{|c||}{AR: Pairwise}  & \multicolumn{2}{|c||}{AR: Graph} & \multicolumn{3}{|c||}{MR: Pairwise} & \multicolumn{3}{|c||}{MR: Graph} \\
	\hline
	Dataset &
	    $\gamma$ & 
		Sink Masked &
		Source Masked &
		Sink Masked &
		Source Masked &
		50\% Mask &
		80\% Mask &
		90 \% Mask &
		50\% Mask &
		80\% Mask &
		90 \% Mask &
		\hline 
	COPD &
		0.000 &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
	&
		0.001 &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
	&
		0.005 &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		\hline 
	Census &
		0.000 &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
	&
		0.001 &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
	&
		0.005 &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		\hline 		
	IMDB &
		0.000 &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
	&
		0.001 &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
	&
		0.005 &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		\hline 
		
	CIFAR10 &
		0.000 &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
	&
		0.001 &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
	&
		0.005 &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		\hline 
		
		
		

	\hline
\end{tabular}
\caption{Caption}
\label{table:AR}
\end{table*}



==> tables/table_redundancy_v2.tex <==




\begin{table*}[t]
\scriptsize
\centering
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{|c||c|c||c|c||c|c||c|c||c|c||c|c||c|c||}
    \hline
    & \multicolumn{2}{|c||}{COPD}  &
    \multicolumn{2}{|c||}{MNIST}  &
    \multicolumn{2}{|c||}{CIFAR10}  &
    \multicolumn{2}{|c||}{IMDB}  &
    \multicolumn{2}{|c||}{Census}  &
    \multicolumn{2}{|c||}{Divorce}  &
    \multicolumn{2}{|c||}{Drug} \\
	\hline
	    $\gamma$ & 
		Source &
		Sink &
		Source &
		Sink &
		Source &
		Sink &
		Source &
		Sink &
		Source &
		Sink &
		Source &
		Sink &
		Source &
		Sink &
		\hline 
		
	0.000 &
		100.0 &
		63.9 &
		100.0 &
		12.8 &
		99.6 &
		12.6 &
		87.5 &
		48.0 &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &

	0.001 &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &

	0.005 &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &
		-- &

		\hline 

	\hline
\end{tabular}
\caption{Comparison of masking sink and source nodes of graph $\mathcal{H}$, where sink nodes represent directionally redundant features.}
\label{table:AR}
\end{table*}



==> tables/table_redundancy_v3.tex <==


\begin{table*}[t]
\scriptsize
\centering
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.3}
        \begin{tabular}{| c | p{0.7cm} p{0.7cm} | p{0.7cm} p{0.7cm} | p{0.7cm} p{0.7cm} | p{0.7cm} p{0.7cm} |}
            \hline
            & \multicolumn{4}{|c|}{PH-Accy}  & 
            \multicolumn{4}{|c|}{\% Feat Masked} \\
            
            \hline
            & \multicolumn{2}{|c|}{PH-Accy}  & 
            \multicolumn{2}{|c|}{\% Feat Masked} &
            \multicolumn{2}{|c|}{PH-Accy}  & 
            \multicolumn{2}{|c|}{\% Feat Masked} \\
            
        	\hline
        		
            	Dataset &
        		Sink Masked & 
        		Source Masked &
        		Sink Masked & 
        		Source Masked &
        		Sink Masked & 
        		Source Masked &
        		Sink Masked & 
        		Source Masked &
        		
            	\hline
            	
            	COPD &
        		99.5&
        		62.7&
        		1.5 &
        		98.5 &
        		
        		-- &
        		-- &
        		-- &
        		-- &
        		
            	CIFAR10 &
        		94.6 &
        		15.0 &
        		6.2 &
        		93.8 &
        		
        		-- &
        		-- &
        		-- &
        		-- &
        		
            	MNIST &
        		100.0 &
        		13.4 &
        		77.7 &
        		22.3 &
        		
        		-- &
        		-- &
        		-- &
        		-- &
        		
            	IMDB &
        		100.0 &
        		54.0 &
        		3.5 &
        		96.5 &
        		
        		-- &
        		-- &
        		-- &
        		-- &
        		
            	Census &
        		100.0 &
        		82.0 &
        		23.8 &
        		76.2 &
        		
        		-- &
        		-- &
        		-- &
        		-- &
        		
            	Divorce &
        		100.0 & 
        		51.5 & 
        		22.2 & 
        		77.8 & 
        		
        		-- &
        		-- &
        		-- &
        		-- &
        		
            	Drug &
        		100.0 & 
        		48.5 & 
        		43.5 & 
        		56.5 & 
        		
        		-- &
        		-- &
        		-- &
        		-- &
        
        	\hline
        \end{tabular}
      
        \caption{Posthoc-accy of BivShap-S after masking $\mathcal{H}$-source nodes, representing features with minimal redundancies, and $\mathcal{H}$-sink nodes, representing directionally redundant features.}
        \label{table:directional_redundancy}
\end{table*}


==> tex/experiments.tex <==
\section{Experiments}\label{sec:experiments}

In this section, we investigate the ability of Bivariate Shapley for discovering (1) mutual redundancy, (2) directional redundancy, and (3) influential features, from black-box models.
%======================================================

%\subsection{Experiment Setup.}

\textbf{Test Settings.}
%In this section, we investigate the validity of directional feature interaction. 
%We evaluate our two introduced notions of redundancy, \emph{Mutual Redundancy} and \emph{Directional Redundancy}, identified on the $\mathcal{H}$ graph and $\mathcal{G}$ graph.
We apply Bivariate Shapley on seven black-box models trained on different datasets.
We take $500$ test samples from each dataset (less if the test set is smaller than $500$) and generate their respective $\mathcal{G}$ and $\mathcal{H}$ graphs.
We select $\gamma = 10^{-5}$ for the threshold in converting $\mathcal{G} \rightarrow \mathcal{H}$, which generally corresponds to $50\%$ average graph density across the datasets (see App. \ref{app:experiments} for details).
%Shapley value methods generally require a choice of a baseline value, which represents the value of unselected or removed features. For tabular data, we define this value to be zero, except the Divorce dataset where a value of `3' indicates the average response.  For images, we use a pixel value of zero. For text, we set the word embedding for the selected feature to be the zero vector.
All experiments are performed on an internal cluster equipped with Intel Gold 6132 CPUs and Nvidia Tesla V100 GPUs. The source code will be made publicly available at \url{https://github.com/davinhill/BivariateShapley}.

\textbf{Evaluation Measure.} We evaluate mutual and directional redundancy using post-hoc accuracy \citep{pmlr-v80-chen18j}, where the redundant features in a set of samples are masked, and accuracy is evaluated between the masked samples and original predictions. During masking we replace the selected feature with a baseline value which represents feature unavailability. We also evalute influential features using insertion and deletion AUC \citep{petsiukrise}. dAUC iteratively removes the highest-ranked features of a given image and measures the change in model output compared to the baseline prediction, as summarized by the area under the curve. iAUC starts with an uninformative baseline sample then iteratively inserts the highest-ranked features, then similarly measures change in model output.

\textbf{Datasets and Models.}
We evaluate our methods on a $1077$ RNAseq COPDGene data~\citep{reganGeneticEpidemiologyCOPD2010}, CIFAR10~\citep{Krizhevsky09learningmultiple} and MNIST~\citep{lecun-mnisthandwrittendigit-2010} image data, IMDB~\citep{maas2011learning} movie review text data, and on three tabular UCI datasets (Drug, Divorse, and Census)~\citep{Dua:2019}. We train separate black-box models for each dataset. Image and text datasets, as well as COPDGene and Divorce use neural network architectures; Census and Divorce use tree-based models (XGBoost~\citep{chenXGBoostScalableTree2016} and Random Forest). Full dataset details and model settings can be found in App. \ref{app:experiments}.

\begin{comment}
\begin{itemize}
    \item \textbf{Genetic.} We use a 1,077 gene subset of the COPDGene dataset to investigate differences in gene interaction between smokers and nonsmokers. We use a Multi-Layer Perceptron (MLP) with 4 hidden layers each with 200 hidden units, relu activation, and batch normalization.
    \item \textbf{Image.} We use the classic image classification datasets CIFAR10 and MNIST. We follow Ribeiro et al. \citep{ribeiro2016should} in using superpixels; this reduces computational cost and improves the interpretability of selected pixels. We use 196 and 255 superpixels for MNIST and CIFAR10, respectively, using \emph{simple linear iterative clustering} \citep{achantaSLICSuperpixelsCompared2012} with smoothing parameter $\sigma = 5$. For CIFAR10 we use also use  standard data augmentations consisting of random horizontal flips and color jittering.
    \item \textbf{Text.} we use the IMDB movie review dataset for sentiment analysis. In order to improve accuracy, we initialize the model word embedding with GloVe pretrained features \citep{pennington2014glove}
    \item \textbf{Tabular.} Drug, Divorce, and Census are UCI datasets \citep{Dua:2019}. In Drug, we predict whether an individual will consume the drug LSD, given reported consumption habits of 6 other drugs. In Divorce, we use questionnaire responses to predict divorce. Census uses the 1996 census database; we predict whether an individual has annual income greater than $\$50K$ given basic demographic data.
\end{itemize}
\end{comment}

%\input{tables/table_datasets}



\textbf{Competing Methods.} 
We compare our method against both univariate and bivariate, instance-wise, black-box explanation methods. Univariate methods Shapley sampling values \citep{vstrumbelj2014explaining}, Kernel SHAP \citep{NIPS2017_8a20a862}, L2X~\citep{pmlr-v80-chen18j} are used to identify the top important features, either through a feature ranking or by choosing a subset of features. Second-order methods Shapley Interaction Index \citep{shapley_interaction}, Shapley-Taylor Index \citep{sundararajanShapleyTaylorInteraction2020}, and Shapley Excess capture symmetric interactions, for which we apply the same PageRank algorithm as Bivariate Shapley to derive a feature ranking.
Further details regarding control parameter settings of these competing methods and licensing information are provided in App \ref{sec:experiment_setup}.

\begin{comment}
\begin{itemize}
    \item \textbf{Shapley sampling values} \citep{vstrumbelj2014explaining} uses Monte Carlo sampling to approximate Shapley values. Since we use this algorithm to compute Bivariate Shapley, we can calculate the univariate Shapley values concurrently.
    \item \textbf{Kernel SHAP} \citep{NIPS2017_8a20a862} is another approximation method for Shapley values, which uses a linear explanation model to locally approximate the black box.
    \item \textbf{L2X} \citep{pmlr-v80-chen18j} trains an explainer model that minimizes the mutual information between the selected features and the labels. We use a 5-layer MLP for the tabular, text, and genetic datasets and a 5-layer CNN for the image datasets. We then train a separate explainer model for each chosen masking subset for our tests.
    \item \textbf{Shapley interaction values} \citep{shapley_interaction} is a second-order extension to Shapley values, which separates feature interactions and main effects. We apply the tree-based algorithm introduced by Lundberg et al. \citep{lundbergConsistentIndividualizedFeaturea}, and use the Kernel SHAP approximation to calculate interaction values for other model types.
\end{itemize}
\end{comment}

%=================================================
%\subsection{Building Graphs \mathcal{G} and \mathcal{H}}




%Since each feature within the group provides redundant information with respect to the label, masking other features within the group should have minimal impact to accuracy.
%=================================================
\textbf{(1) Mutual Redundancy Evaluation.}

\begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth]{figures/MR.pdf}
\end{center}
   \caption{Post-Hoc Accuracy (higher is better) evaluated on Mutual Redundancy and Directional Redundancy derived from graph $\mathcal{H}$. Note that Shapley-Taylor and Shapley Excess methods are only evaluated on the smaller datasets Divorce, Drug, and Census due to computational complexity. Strongly connected nodes in $\mathcal{H}$ are randomly masked with increasing mask sizes until a single node remains, represented by the final marker for each dataset.}
\label{fig:MR}
\end{figure}



We evaluate the validity of mutually redundant features by evaluating the change in model accuracy after masking redundant features, with results shown in Figure~\ref{fig:MR}(a). We identify such features as groups of strongly connected nodes in graph $\mathcal{H}$, which we find using a depth-first search on $\mathcal{H}$ using Tarjan's algorithm \citep{Tarjan1972DepthFirstSA}. After finding the mutually redundant groups, we test their exchangeability by randomly selecting subsets of features within the group to mask. We evaluate post-hoc accuracy at different levels of masking. Masking all but one feature results in the quotient graph $\mathcal{S}$, which is represented by each dataset's marker in Figure~\ref{fig:MR}(a). Note that these groups can be discovered by other second-order methods by similarly interpreting the resulting feature interactions as an adjacency matrix; we include the results for applying the same algorithm to Shapley interaction values.
%
%
\input{tables/table_TimeComplexity}
We observe in Figure~\ref{fig:MR}(a) that masking an arbitrary number of mutually redundant features has minimal impact to accuracy under the Bivariate Shapley method. In contrast, the groups identified by Shapley interaction values do not share the same level of feature interchangeability. In terms of finding mutual redundancy, this suggests that incorporating directionality is critical in identifying mutually redundant features. Undirected methods do not capture the full context of feature interactions. 
%
We also observe different patterns of mutual redundancy between the datasets. Collapsing the entirety of mutually redundant groups in MNIST results in masking $80\%$ of total features, indicating high levels of redundancy. Examples in Figure~\ref{fig:MR}(a) demonstrate that these groups represent background pixels unrelated to the label. However, datasets such as COPD and CIFAR10 only exhibit $2\%$ and $3\%$ mutually redundant features, which implies that their features are not similarly interchangeable.


%=================================================
% Directional Redundancy
\textbf{(2) Directional Redundancy Evaluation.}
We similarly validate directional redundancy using post-hoc accuracy, as seen in figure~\ref{fig:MR}(b).We identify directionally redundant features as $\mathcal{H}$-sinks and $\mathcal{H}$-sources, which we identify using PageRank. We collapse the strongly connected components in graph $\mathcal{H}$ to its quotient graph $\mathcal{S}$, then apply PageRank to each connected graph in $\mathcal{S}$. The maximum and minimum ranked nodes in each connected graph correspond to the sinks and sources in $\mathcal{S}$, respectively. The condensed sinks and sources are expanded to form $\mathcal{H}$-sinks and $\mathcal{H}$-sources. We then evaluate the relevance of the identified nodes using post-hoc accuracy of masked samples. To validate our claims of directionality, we compare the results of masking $\mathcal{H}$-source nodes and $\mathcal{H}$-sink nodes, where $\mathcal{H}$-sink nodes represent the directionally redundant features. We observe that masking sinks have little effect on accuracy, suggesting that these features contain redundant information given the unmasked source nodes. In contrast, masking source nodes and keeping sinks results in large decreases in accuracy, indicating that prediction-relevant information is lost during masking.


%=================================================
\textbf{(3) Influential Feature Evaluation.}
While mutual and directional redundancy can be investigated individually using graph $\mathcal{H}$, we can combine both concepts in a continuous ranking of features based on the steady-state distribution of a random walk on graph $\mathcal{G}$. We add a small $\epsilon \approx 0$ value to the adjacency matrix of $\mathcal{G}$ to ensure that all nodes are connected, then directly apply PageRank. The resulting feature scores are ranked, with high-scoring features representing high importance. 
%
We observe the experiment results in Figure \ref{fig:main_comparison}. Bivariate Shapley outperforms the other second-order method, Shapley interaction values, as well as most univariate methods, while being competitive with Shapley Sampling. Note that Bivariate Shapley does not explicitly utilize feature importance, but rather each feature's steady-state distribution. However we can also incorporate feature importance information, defined by univariate Shapley, through Personalized PageRank. Personalization increases the steady state probabilities for important features.


\begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth]{figures/main_comparison.pdf}
\end{center}
   \caption{Comparison of explanation methods on a feature removal task. We apply PageRank to graph $\mathcal{G}$ to derive a univariate ranking based on feature redundancy. We compare to popular explanation methods by iteratively masking the lowest ranked features. Shapley sampling values, Kernel SHAP, L2X are univariate methods; Interaction shapley (Int) is a second-order method where we apply the same PageRank metholodology for comparison.}
\label{fig:main_comparison}
\end{figure}


\input{tables/table_AUC}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Time Complexity
\textbf{(4) Time Complexity Evaluation}
Note that while we primarily investigate Shapley-based methods, our method can be generalized to any removal-based explainer, as mentioned in Section~\ref{uni_to_multi}. More concretely, each column of the $d \times d$ adjacency matrix, representing interactions between d features, can be considered an independent explanation where the column feature is always present. Therefore our method is extremely flexible; the user can decide which explanation method to use based on the constraints of their intended application. It follows that our method’s time complexity is dependent on the choice explanation method and, when implemented naively, linearly scales that method’s complexity by the number of features. Certain methods, such as KernelSHAP, can be adapted to realize even more efficient implementations of Bivariate Shapley, which we outline in App~\ref{sec:alg}. We provide time comparisons to competing methods in Table~\ref{table:time}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% COPD

\input{tables/table_COPD}

\textbf{Gene Ontology Enrichment Analysis of COPDGene Dataset} Chronic Obstructive Pulmonary Disease (COPD) is a chronic inflammatory lung disease representing the $4^{\text{th}}$ leading cause of death  \citet{TechnicalNotesSummary} in the United States. The relation between COPD and smoking is well-established; It has been shown
smoking enhance the risk of getting lung disease through variety of way such increasing inflammation \citep{arnson2010effects}.
In this paper, we investigate the relation between gene expression data and Smoking status (Smoking and non-smoking prediction) in COPDgene data. We show the interpretation power of our methods, by relating our most influential genes to biological pathways which correspond to smoking. In particular, we performed
Gene Set Enrichment Analysis (GSEA) using the GenePattern web interface \footnote{\url{https://cloud.genepattern.org/gp/pages/index.jsf}} on the ranking of influential features.

We generate this ranking of influential features as follows. We first calculate graph $\mathcal{G}$ for each test sample, as in Alg.~\ref{alg:G}. We then create the global $\mathcal{G}$ graph for each subgroup, smokers and non-smokers, by averaging the $\mathcal{G}$ adjacency matrix over all samples within each subgoup (figure~\ref{fig:COPD_G}). We can then directly apply the ranking algorithm outlined in section~\ref{sec:alg} to obtain importance scores for the features within each subgroup.

We use the list of 1,079 unique gene names with their associated importance score as input into the GenePattern interface. Gene set enrichment for these two groups was calculated using the GSEAPreranked module with 1000 permutations, using the Hallmark (h.all.v7.4.symbols.gmt) and Immunologic gene sets (c7.all.v7.4.symbols.gmt). Pathways with a q-value less than 0.05 are reported as significant according to the recommendation of the developers \footnote{\url{http://www.gsea-msigdb.org/gsea/doc/GSEAUserGuideTEXT.htm#_Interpreting_GSEA_Results}}. 
We observed 
pathways corresponding to Macrophages. Macrophages are types of immune cells, which can initiate inflammation. 
They also involve in detection and destruction of bacteria in the body. 
The relation between such cells and smoking has been observed in biological domain, in many studies it has been observed that smoking induces changes in the immune cell function in COPD patients \citep{yang2018cigarette,strzelak2018tobacco}, the complete table of Pathways is in Table~\ref{table:COPD}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Illustrative Examples

\subsubsection{Additional Illustrative Examples from MNIST, CIFAR10, and IMDB Data} \label{app:experiments}

\begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth]{figures/Examples.pdf}
\end{center}
   \caption{We explore samples from MNIST, CIFAR10, and MNIST. Center column: we identify Mutually Redundant features from graph $\mathcal{H}$, indicated by the white pixels in each image and text highlights. Right column: We apply redundancy ranking on graph $\mathcal{G}$ and show a heatmap of PageRank scores; the most important nodes have higher PageRank scores, indicated by lighter pixels in the heatmap. For IMDB, we highlight the top-5 highest-scoring features.}
\label{fig:examples}
\end{figure}

In Figure~\ref{fig:examples} we investigate a number of examples from MNIST, CIFAR10, and IMDB results for illustrative purposes. 
The left column is the original data.  The center column displays the mutually redundant features indicated by the white pixels in each image and yellow highlights for text data.  The right column shows heatmaps of PageRank scores (the higher the scores, the more important the features).  For IMDB data, the top-5 highest ranking scores are highlighted in red.
All redundancy calculations use the same parameters as in our previous experiments, except for calculating mutual redundancy on IMDB for which we use $\gamma = 1e-3$ to capture additional redundant features. 

For the image examples, we see that images with homogenous background pixels show larger amounts of redundancy as identified using graph $\mathcal{H}$ in the center column. This redundancy is also evidenced in the directional redundancy ranking in the right column, where the mutually redundant pixels are shown to have similar PageRank scores.  We observe that pixels with higher scores make sense and correspond to pixels where the foreground object lies in the image and at key areas of the object.  Similarly, the top 5 words selected on the right column for IMDB are relevant words for predicting the rating of the movie.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DOMAIN ANALYSIS OF RESULTS

\iffalse
\textbf{Domain Analysis of Results.}
%=================================================
{\bf COPD} is a chronic inflammatory lung disease related to smoking. 
We performed a Gene Set Enrichment Analysis using GenePattern~\citep{reich2006genepattern} on the ranking of influential features obtained by Bivariate Shapley.  Details of the analysis and results are in App.~\ref{app:experiments}.
The results show that the most important pathway discovered
correspond to macrophages, which are types of immune cells, which can initiate inflammation. 
%They also involve in detection and destruction of bacteria in the body. 
%
{\bf IMDB.} Fig.~\ref{fig:Univariate shapley versus Shapley Graph} provides an example directed explanation graph for an instance of the IMDB data.  Additional examples are reported in App.~\ref{app:experiments}.

\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


